Teaching Shortest Path Algorithms With a Robot and Overlaid Projections

Robots have the potential to enhance teaching of advanced computer science topics, making abstract concepts more tangible and interactive. In this paper, we present Timmy-a GoPiGo robot augmented with projections to demonstrate shortest path algorithms in an interactive learning environment. We integrated a JavaScript-based application that is projected around the robot, which allows users to construct graphs and visualise three different shortest path algorithms with colour-coded edges and vertices. Animated graph exploration and traversal are augmented by robot movements. To evaluate Timmy, we conducted two user studies. An initial study (n=10) to explore the feasibility of this type of teaching where participants were just observing both robot-synced and the on-screen-only visualisations. And a pilot study (n=6) where participants actively interacted with the system, constructed graphs and selected desired algorithms. In both studies we investigated the preferences towards the system and not the teaching outcome. Initial findings suggest that robots offer an engaging tool for teaching advanced algorithmic concepts, but highlight the need for further methodological refinements and larger-scale studies to fully evaluate their effectiveness.

==> Ch3_user_studies.tex <==
\par We run two user studies: an initial user study and a pilot user study. %The initial user study was carried out early in the research, while the pilot user study took place at the end.
The initial user study aimed to address two primary questions: 

\begin{enumerate}[noitemsep]
    \item \textbf{Effectiveness of the GoPiGo Robot:} Can the GoPiGo robot effectively serve as a tool for teaching individuals about Dijkstra’s shortest path algorithm?
    \item \textbf{Preference of Learning Method:} Do individuals prefer learning with the robot compared to learning just from a screen?
\end{enumerate}

\par Additionally, this study assessed the robot’s efficiency as an instructor and explored the cognitive demands associated with learning from the robot. The findings from these observations were intended to evaluate the feasibility and potential value of the research.

\par The pilot user study was designed to evaluate the readiness of the final prototype for extensive testing. It focused on identifying any shortcomings in the prototype. Assessing the user enjoyment with the application, as well as comparing user preferences between the robot-based and the screen-based learning. The study examined how users interacted with the graph-drawing application and managed the robot or screen conditions. The goal was to determine how well the final prototype was prepared for the next stages of development.


\section{Initial User Study}

\par This study was conducted using the initial version of the system (see \autoref{sec:initial_version}). It involved 10 participants (\textbf{I\_P01}--\textbf{I\_P10}) aged 18 to 25, all with prior knowledge of graph theory. The study was conducted in a controlled environment. It featured two conditions: screen condition and a robot condition. Participants were split into two groups. Half begun with the screen condition, and the other half with the robot condition. After reading and signing the consent form participants had a tutorial for the first condition, completed the NASA TLX questionnaire and a short task implementing the Dijkstra’s Shortest Path algorithm on a different graph. The same procedure (tutorial, NASA TLX and the task) was held for the second condition.

\par During each tutorial, participants learned about Dijkstra’s Shortest Path algorithm. As explained earlier the interface displayed (i) the pseudo code for the algorithm on the left side of the screen (\autoref{fig:screenConditionGraph}), (ii) distance, and (iii) predecessor updates on the right side. In the canvas in the middle there was a pre-drawn graph. Participants observed the graph without direct interaction. They received introduction to what they were seeing on the screen. They were allowed as much time as needed to review the graph before proceeding.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.8\textwidth]{Chapters/Images/FinalScreenConditionGraph.png}
  \caption{Final view of the Graph in the Screen Condition. The shortest path is visualised in red colour.}
  \label{fig:screenConditionGraph}
\end{figure}

\par In the screen condition, participants observed the algorithm’s execution with the final shortest path highlighted with red edges. In the robot condition, participants observed the same graph exploration process, but without the final path highlighted. Instead, the robot traversed the path, demonstrating the final shortest path determined by Dijkstra’s algorithm. 

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/ScreenConditionTesting.png}
        \caption{Screen condition testing graph.}
        \label{fig:screenConditionTest}
    \end{subfigure}
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/RobotConditionTesting.png}
        \caption{Robot condition testing graph.}
        \label{fig:robotConditionTest}
    \end{subfigure}
    \caption{Testing graphs for the two conditions.}
    \label{fig:testingGraphs}
\end{figure}

\par The task after each condition involved the implementation of the Dijkstra’s Shortest Path algorithm on another graph. Two graphs shown in \autoref{fig:testingGraphs} were used, one for each condition. The graph structure was the same as in tutorials and for both tasks just the edge weights varied. 
The study provided feedback on whether participants can learn from either condition and are able to implement Dijkstra’s Shortest Path algorithm following the tutorials. %By dividing the participants to different start conditions, the study aimed to offer deeper insights into the relative effectiveness of each condition. As well as the impact of the condition on the participants abilities to implement the algorithm.

\section{Pilot User Study}

\par The pilot study was conducted using the final version of the system (see \autoref{sec:final_version}), and involved 6 participants (\textbf{P\_P01}--\textbf{P\_P06}) aged 21 to 23 in a controlled environment.

\par As in the initial study, there were two conditions. The screen condition and the robot condition. Participants were divided equally, with half starting with the screen condition and the other half starting with the robot condition. In the screen condition, participants observed the algorithms solely on screen. In the robot condition, participants watched the robot demonstrate the algorithms using various gestures as seen in \autoref{fig:observingTheRobot}. 

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/participantObservingRobot1.jpg}
    \end{subfigure}
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/participantObservingRobot2.jpg}
    \end{subfigure}
    \caption{Participants observing the robot.}
    \label{fig:observingTheRobot}
\end{figure}

\par Participants first read and signed the consent form. They were then introduced to the graph drawing application. After being introduced to all of the features of the application they were given time to familiarise with it (\autoref{fig:participantAppInteraction}). Once comfortable with the application, participants were tasked with drawing a graph with 6 vertices. This was done to ensure consistency in difficulty in the graphs over all participants. If the researcher determined that a participant’s graph was too simple (in terms of edge count), they were asked to add additional edges to vertices of their choice. Once participants were satisfied with their graph, they began the learning process.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.6\textwidth]{Chapters/Images/participantInteractingWithApplication.jpg}
  \caption{Participant interacting with the graph drawing application.}
  \label{fig:participantAppInteraction}
\end{figure}

\par Participants had the option to access pseudo code for the algorithms. This was possible at any time before and after viewing the algorithms. They used the application to view the algorithms being demonstrated. Clicking buttons corresponding to each algorithm and condition. The algorithms were shown in the following order: Dijkstra’s, A* (A Star), and Bellman-Ford. The process was the same for both conditions. The only difference being that participants in the robot condition received also instructions on how to interact with the robot properly.

\par For each condition after going through all of the algorithms, participants were tasked with filling out a SUS (System Usability Score) questionnaire \autoref{appendix:sus}. Upon completing the second condition, they were also asked to fill out the final user questionnaire (\autoref{appendix:pilot_questionnaire1}).








==> Ch4_results.tex <==
\section{Initial User Study results}
\subsection{NASA-TLX Mental Workload Results}

\par Based on the results of the NASA TLX tests, it appeared that the screen condition imposes slightly less mental demand compared to the robot condition (see \autoref{fig:cognitiveLoads}). However, since both conditions recorded average overall loads around 20\%, there was a room for improvement and potential increasing the information load provided to the user.

\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/CognitiveLoadScreenCondition.png}
        \caption{Cognitive load of the screen condition.}
        \label{fig:cognitiveLoadScreen}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Chapters/Images/CognitiveLoadRobotCondition.png}
        \caption{Cognitive load of the robot condition.}
        \label{fig:cognitiveLoadRobot}
    \end{subfigure}
    \caption{Cognitive loads of both conditions.}
    \label{fig:cognitiveLoads}
\end{figure}

\subsection{Evaluation of Algorithm Implementation Results}

\par The majority of participants in the initial user study encountered challenges in effectively implementing the Dijkstra’s Shortest Path algorithm. Even though they received tutorials on how the algorithm works. Surprisingly, participant I\_P09 was the only individual who actively read and accurately followed the pseudo code. Others, such as I\_P02, I\_P04 and I\_P08, attempted the implementation but omitted crucial steps, resulting in incorrect solutions. Participants I\_P01, I\_P06, and I\_P10 opted for Prim’s algorithm instead of Dijkstra’s, where I\_P10 neglected to consider alternative paths and selected the first solution as final. Participants I\_P05, I\_P08, and I\_P09 were successful in implementing the algorithm. However, participant I\_P08 missed a crucial relaxation step in the screen condition which led to the wrong answer.


\subsection{Initial User Questionnaire Results}

\par The user questionnaire (see \autoref{appendix:initial_questionnaire1}) revealed unanimous preference for the robot over the screen among all participants. Moreover, the majority of participants expressed a belief that learning from the robot was more effective for understanding shortest path algorithms. Interestingly, opinions were divided on which platform was easier to handle. Some participants favoured the screen and others found the robot more manageable.

\par Notably, some of the participants, namely I\_P04, I\_P06, and I\_P10, answered that they would recommend the robot to their colleagues. They also expressed a desire for teachers to incorporate robot-based methods into the classroom instructions. However, the majority of participants favoured both the screen and robot, suggesting a balanced perspective on effectiveness of each platform. 

\subsection{Overall Results}

\par The findings from the initial user study demonstrated significant potential for integrating robotics into the education system. However, it is crucial to refine the methods used to ensure their effectiveness. The study highlighted the importance of providing diverse learning options to fit individuals preferences and learning styles. Offering a variety of educational tools and approaches can better meet the needs of each student.


\section{Pilot User Study Results}
\subsection{SUS Test Results}

\par The SUS test results indicate that both the screen and the robot conditions have similar usability scores. Both of them going above the average range. However, the screen condition was rated higher than the robot condition, with a difference of around 7.5 points. The average scores and standard deviations for each condition as seen on the \autoref{fig:susScoresParticipants} are:

\begin{itemize}
    \item Screen Condition
    \begin{itemize}
        \item Average Score: 80.42
        \item Standard Deviation: 8.34
    \end{itemize}
    \item Robot Condition
    \begin{itemize}
        \item Average Score: 72.92
        \item Standard Deviation: 6.02
    \end{itemize}
\end{itemize}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{Chapters/Images/SUS-scores.png}
  \caption{Overall SUS scores across participants.}
  \label{fig:susScoresParticipants}
\end{figure}

\subsection{Pilot User Questionnaire Results}

\par The questionnaire is available in \autoref{appendix:pilot_questionnaire1}. For the question \textbf{Q1}, which asked participants whether they preferred the screen or the robot, the responses were nearly evenly split. With only one more participant favouring the robot. Participant P\_P06 explained that their preference for the screen was due to the speed at which information was presented. They noted that the screen condition was significantly faster than the robot and helped maintain their focus better.

\par Question \textbf{Q2} asked participants which method they believed was better for teaching shortest path algorithms. The screen condition was preferred over the robot, with a score 4 to 2. Participants P\_P01 and P\_P02 favoured the robot. They said that it was visually engaging and easier for them to understand the algorithm, as well as helped maintaining their attention. That was not the case for participant P\_P04 as they found the robot too distracting and preferred a more straightforward approach. Stating ``The more boring the better for me.'' Participant P\_P05 noted that the screen was more efficient time-wise. Meanwhile, participant P\_P06, while choosing the screen, suggested that an ideal approach would combine both methods.

\par Question \textbf{Q3} asked which method participants believed would be better for teaching shortest path algorithms to primary school children. All participants chose the robot. Many noted that the robot would be more engaging and enjoyable for children. Making them more likely to stay focused and interested in the learning process. 

\par Question \textbf{Q4} asked which method participants found easier to handle. Four participants preferred the robot. While two participants had no strong preference and chose both methods. Participant P\_P01 explained their preference for the screen, noting that it required less handling ``Just clicking a button.'' compared to the robot.

\par Question \textbf{Q5} asked which method participants would recommend to their colleagues. All participants chose to recommend both the screen and the robot. Some participants mentioned that the choice should depend on individual preferences and tastes. As both methods can be suited to different learning styles.

\par Question \textbf{Q6}, asked whether participants would like to have the robot as a tool for learning algorithms in general. All participants answered ``Yes''. Participant P\_P01 mentioned that the robot would make learning more interesting. Participant P\_P02 added that, as technology advances, there will likely be more tools like this.

\par In the open comments, participants offered several suggestions for enhancing the user interface and overall experience. Participants P\_P01 and P\_P02 both recommended adding two buttons to enable switching between modes as this would, in their opinion, improve the UI and user experience. Participant P\_P01 also suggested clarifying when the robot starts ``drawing'' the shortest path. Participant P\_P02 requested faster transitions on the screen method. Participant P\_P05 proposed using a smaller robot to reduce costs and make it more suitable for personal use. Participant P\_P06 mentioned difficulty maintaining attention while using the robot and suggested that colouring the lines could make it easier to track progress. They recommended using a grey colour for edges that are explored in the current iteration and marking edges that will not be revisited.

\subsection{Overall}

\par The pilot study findings demonstrate that user preference for educational methods depends significantly on their preference. Both the screen and robot are generally usable. Enhancing the robot’s usability to match or surpass the screen’s performance could improve its effectiveness. Users show diverse preferences for both methods, with the robot being manageable but requiring simpler operation for better accessibility. There is strong interest in using robots for educational purposes. Suggesting that ongoing development and integration of robotic tools in learning environments could be highly beneficial.

==> Ch6_discussion.tex <==
\par Numerous studies have explored the integration of robotics into education. Focusing primarily on teaching robotics or using robots for general educational purposes. This thesis investigates whether robots are suitable as teaching tools for more complex topics. To be exact it investigates whether a robot, namely the GoPiGo, is suitable for more clearly explaining the shortest path algorithms. While the GoPiGo is a solid choice for beginners in robotics, it presents challenges for more advanced applications like the one  presented in this research. The GoPiGo has several limitations that may make it less ideal for specialised projects. Consequently, alternative robots might be better suited for this kind of research.

\par Regarding the potential of robots as educational tools, the first study conducted in this research suggest a preference for using robots in teaching. However, effectiveness largely depends on how the teaching method is implemented and user preferences. %After the pilot study we saw that the method affects users preference. Whether users interact directly with the robot or merely observe it. 
In the initial study when users would only observe the robot traversing the pre-built graph, they preferred it more. When they had to built the graphs on their own and interact with the robot in the pilot study, they were more prone to choose the screen condition as a preferred one. 

\par Despite the small sample sizes in the studies (10 participants in the initial user study and 6 in the pilot study) there is evidence suggesting potential for further exploration in this field. To fully asses this potential, further extensive testing is required. One limitation in this study is also the age of participants who might not be the best target audience. The inclusion of younger participants would also be necessary. 

==> Ch7_conclusion.tex <==
\par This thesis explored whether a robot, specifically the GoPiGo robot, can effectively serve as teaching tools for complex subjects such as shortest path algorithms. The idea was that with a physical robot traversing the graphs and searching for the shortest path, users might be better at grasping the intricacies of different shortest path algorithms. The study examined three algorithms: Dijkstra’s, A* (A Star) and Bellman-Ford.

\par The research involved developing a teaching environment. The GoPiGo was paired with a graph drawing application projected onto a flat surface. Initially, the robot and application operated separately. The drawn graph was manually inputted into the robot. However, following upgrades to both the robot’s OS and the application, direct integration was achieved. This allowed automatic graph feeding and robot control from the application.

\par Two user studies were conducted. One with the initial setup and one with the upgraded system. Despite the small sample sizes (10 participants in the initial study and 6 in the pilot study), the findings indicated a potential for using robots in education. The studies revealed that the robot generally maintained user’s attention. However, participants preferred the robot condition in the initial study more than in the pilot study. This shows that the teaching method affects learning preference. Effective instructional strategies are thus crucial to fully leverage the robot’s capabilities in educational settings.

\par To fully explore the potential of robots teaching complex subjects, a more extensive research that focuses on improving instructional approaches and optimising the use of robots as teaching tools is needed. In addition, different age groups should be involved in future studies as well.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
